Case2Flow: Bridging Patient Cases and Guideline Flowcharts through Multimodal Retrieval

Medical guidelines encode rich, evidence-based decision logic, yet the specific decision artifact a clinician needs is hard to locate within a guideline, let alone across guidelines covering plausible diseases and treatments. While guideline passages have supported end-to-end question answering, flowcharts remain largely underused in decision support despite their ability to encode actionable clinical pathways. We therefore introduce Case2Flow, a task designed to retrieve the most relevant guideline flowchart for a given patient case from a collection of guideline documents. To support it, we construct FlowAtlas, a curated corpus of 202 flowcharts extracted from 2,080 medical guidelines, together with a pipeline that synthesises 1,911 aligned case-flowchart pairs. Our evaluation of multimodal retrieval methods reveals systematic failure modes, including overreliance on keywords and spurious token-patch matches induced by uninformative background regions in flowcharts. Motivated by this, we propose CRISP, a training-free scoring method that sharpens late-interaction retrieval by suppressing uninformative patches, discounting ambiguous token matches, and incorporating bidirectional query-image alignment. CRISP improves Recall@1 by up to 18.71 percentage points, while a blinded physician assessment on published case narratives provides preliminary feasibility evidence beyond synthetic queries.

==> tables/mixed.tex <==
\begin{table*}[tbp]
    \centering
    \footnotesize
    \renewcommand{\arraystretch}{1.15}
    \setlength{\tabcolsep}{6pt}
    \begin{tabular}{@{} l cccc cccc @{}}
        \toprule
        & \multicolumn{4}{c}{\cellcolor{gray!10}\textbf{\texttt{Original} queries}} & \multicolumn{4}{c}{\cellcolor{gray!40}\textbf{\texttt{Rewritten} queries}} \\
        \cmidrule(lr){2-5} \cmidrule(lr){6-9}
        \textbf{Method} & R@1 & R@5 & R@10 & MRR & R@1 & R@5 & R@10 & MRR \\
        \midrule
        \multicolumn{9}{c}{\textit{Textual Pipeline-Based Flowchart Retrieval}} \\
        \midrule
        OCR + BM25            & \cellcolor{gray!10}62.55 & \cellcolor{gray!10}83.23 & \cellcolor{gray!10}88.75 & \cellcolor{gray!10}71.71 & \cellcolor{gray!40}58.55 & \cellcolor{gray!40}80.90 & \cellcolor{gray!40}86.85 & \cellcolor{gray!40}68.40 \\
        VLM Cap.\ + BM25      & \cellcolor{gray!10}71.83 & \cellcolor{gray!10}91.20 & \cellcolor{gray!10}93.86 & \cellcolor{gray!10}80.50 & \cellcolor{gray!40}68.62 & \cellcolor{gray!40}89.86 & \cellcolor{gray!40}92.97 & \cellcolor{gray!40}78.07 \\
        \midrule
        \multicolumn{9}{c}{\textit{Direct Image-Based Flowchart Retrieval}} \\
        \midrule
        CLIP                  & \cellcolor{gray!10}15.17 & \cellcolor{gray!10}35.78 & \cellcolor{gray!10}46.02 & \cellcolor{gray!10}25.48 & \cellcolor{gray!40}14.73 & \cellcolor{gray!40}34.96 & \cellcolor{gray!40}45.05 & \cellcolor{gray!40}24.85 \\
        Qwen3-VL-Emb          & \cellcolor{gray!10}74.39 & \cellcolor{gray!10}93.95 & \cellcolor{gray!10}96.75 & \cellcolor{gray!10}82.90 & \cellcolor{gray!40}73.05 & \cellcolor{gray!40}93.69 & \cellcolor{gray!40}96.57 & \cellcolor{gray!40}82.03 \\
        ColPali               & \cellcolor{gray!10}55.48 & \cellcolor{gray!10}80.61 & \cellcolor{gray!10}86.43 & \cellcolor{gray!10}66.22 & \cellcolor{gray!40}52.09 & \cellcolor{gray!40}78.44 & \cellcolor{gray!40}84.71 & \cellcolor{gray!40}63.36 \\
        \;+ \textbf{\emph{CRISP}} {\tiny(Ours)} & \cellcolor{gray!10}70.98 & \cellcolor{gray!10}90.00 & \cellcolor{gray!10}93.30 & \cellcolor{gray!10}79.52 & \cellcolor{gray!40}68.23 & \cellcolor{gray!40}87.91 & \cellcolor{gray!40}91.69 & \cellcolor{gray!40}77.16 \\
        ColQwen3              & \cellcolor{gray!10}78.44 & \cellcolor{gray!10}95.15 & \cellcolor{gray!10}97.91 & \cellcolor{gray!10}85.72 & \cellcolor{gray!40}76.93 & \cellcolor{gray!40}94.68 & \cellcolor{gray!40}97.64 & \cellcolor{gray!40}84.68 \\
        \;+ \textbf{\emph{CRISP}} {\tiny(Ours)} & \cellcolor{gray!10}\textbf{83.69} & \cellcolor{gray!10}\textbf{97.62} & \cellcolor{gray!10}\textbf{99.01} & \cellcolor{gray!10}\textbf{89.75} & \cellcolor{gray!40}\textbf{81.88} & \cellcolor{gray!40}\textbf{97.25} & \cellcolor{gray!40}\textbf{98.85} & \cellcolor{gray!40}\textbf{88.56} \\
        \bottomrule
    \end{tabular}
    \caption{Top-$k$ retrieval behaviour on the \emph{Mixed} pool ($257$ candidates across four FlowAtlas sources and the external MedGUIDE/NCCN set). We report Recall@$\{1,5,10\}$ and MRR (\%) for both query modes. CRISP consistently improves all four metrics on both backbones, with the largest gains on R@1 and MRR -- the regimes where ranking sharpness matters most. Best per column in \textbf{bold}. Full per-source Recall@$k$ are in \Cref{sec:full_results}.}
    \label{tab:recall_mixed}
\end{table*}

